FOOGD: Federated Collaboration for Both Out-of-distribution Generalization and Detection

Federated learning (FL) is a promising machine learning paradigm that collaborates with client models to capture global knowledge. However, deploying FL models in real-world scenarios remains unreliable due to the coexistence of in-distribution data and unexpected out-of-distribution (OOD) data, such as covariate-shift and semantic-shift data. Current FL researches typically address either covariate-shift data through OOD generalization or semantic-shift data via OOD detection, overlooking the simultaneous occurrence of various OOD shifts. In this work, we propose FOOGD, a method that estimates the probability density of each client and obtains reliable global distribution as guidance for the subsequent FL process. Firstly, SM3D in FOOGD estimates score model for arbitrary distributions without prior constraints, and detects semantic-shift data powerfully. Then SAG in FOOGD provides invariant yet diverse knowledge for both local covariate-shift generalization and client performance generalization. In empirical validations, FOOGD significantly enjoys three main advantages: (1) reliably estimating non-normalized decentralized distributions, (2) detecting semantic shift data via score values, and (3) generalizing to covariate-shift data by regularizing feature extractor. The prejoct is open in https://github.com/XeniaLLL/FOOGD-main.git.

==> chapters/draft.tex <==



 Stein's Identity and Kernelized Stein Discrepancy Stein's identity plays a fundamental role in our framework. Let $p(x)$ be a continuously differentiable (also called smooth) density supported on $\mathcal{X} \subseteq \mathbb{R}^d$, and $\phi(x)=\left[\phi_1(x), \cdots, \phi_d(x)\right]^{\top}$ a smooth vector function. Stcin's identity states that for sufficiently regular $\phi$, we have
$$
\mathbf{E}_{x \sim p}\left[\mathcal{A}_p \phi(x)\right]=0, \quad \text { where } \quad \mathcal{A}_p \phi(x)=\phi(x) \nabla_x \log p(x)^T+\nabla_x \phi(x),
$$
where $\mathcal{A}_p$ is called the Stein operator, which acts on function $\phi$ and yields a zero mean function $\mathcal{A}_p \phi(x)$ under $x \sim p$. This identity can be easily checked using integration by parts, assuming mild zero boundary conditions on $\phi$, either $p(x) \phi(x)=0, \forall x \in \partial \mathcal{X}^{\prime}$ when $\mathcal{X}^{\prime}$ is compact, or $\lim _{\|x\| \rightarrow \infty} \phi(x) p(x)=0$ when $\mathcal{X}=\mathbb{R}^d$. We call that $\phi$ is in the Stein class of $p$ if Stcin's identity (1) holds.

Now let $q(x)$ be a different smooth density also supported in $\mathcal{X}$, and consider the expectation of $\mathcal{A}_p \phi(x)$ under $x \sim q$, then $\mathbb{R}_{x \sim y}\left[\mathcal{A}_p \phi(x)\right]$ would no longer equal zero for general $\phi$. Instead, the magnitude of $\mathrm{E}_{x \sim q}\left[\mathcal{\mathcal { A } _ { p }} \phi(x)\right]$ relates to how different $p$ and $q$ are, and can be leveraged to define a discrepancy measure, known as. Stein discrepancy, by considering the "maximum violation of Stcin's identity" for $\phi$ in some proper function set $\mathcal{F}$ :
$$
\mathcal{S}(q, p)=\max _{\phi \in \mathcal{F}}\left\{\left[\mathbb{E}_{x \sim \eta} \operatorname{trace}\left(\mathcal{A}_p \phi(x)\right)\right]^2\right\}
$$

Here the choice of this function set $\mathcal{F}$ is critical, and decides the discriminative power and computational tractability of Stein discrepancy. Traditionally, $\mathcal{F}$ is taken to be sets of functions with bounded Lipschitz norms, which unfortunately casts a challenging functional optimization problem that is computationally intractable or requires special considerations (see Gorham and Mackey Ш1] and reference therein).
Kernclized Stein diserepancy bypasses this difficulty by maximizing $\phi$ in the unit ball of a reproducing kernel Hilbert space (RKHS) for which the optimization has a closed form solution. Following Liu
2
et al. [8], KSD is defined as
$$
\mathbb{S}(q, p)=\max _{\phi \in \mathcal{N}^{-.}}\left\{\left[\mathbb{E}_{x \sim \sim}\left(\operatorname{trace}\left(\mathcal{A}_p \phi(x)\right)\right)\right]^2, \quad \text { s.t. } \quad\|\phi\|_{\mathcal{H}^4} \leq 1\right\},
$$
where we assume the kernel $k\left(x, x^{\prime}\right)$ of RKHS $\mathcal{H}$ is in the Stein class of $p$ as a function of $x$ for any fixed $x^{\prime} \in \mathcal{X}^2$. The optimal solution of (2) has been shown $[8-10]$ to be $\phi(x)=\phi_{q, p}^*(x) /\left\|\phi_{q, p}^*\right\|_{H^2}$, where
$$
\phi_{q, p}^*(-)=\mathbb{E}_{x \sim q}\left[\mathcal{A}_p k(x,-)\right], \quad \text { for which we have } \quad \mathbb{S}(q, p)=\left\|\phi_{\psi, p}^*\right\|_{\mathcal{U}^{-t}}^2
$$





Given two probability measures $ \boldsymbol{p}, \boldsymbol{q}$ with observations $\boldsymbol{X}$ and $\boldsymbol{Y}$ respectively, we have $\mathcal{F}$ as a set of functions: $\psi: \mathcal{X} \rightarrow \mathbb{R}$  within a unit ball in the universal Reproducing Kernel Hilbert Space $\mathcal{H}$ (RKHS) with norm $\|.\|_{\mathcal{H}}$.
% 



 \subsection{Stein Variational Gradient Descent}
 Let $p(x)$ and $q(x)$ be a different smooth probability densities supported by $\mathcal{X}$, and 
kernel function in RKHS space $\mathcal{H}$, i.e., $k(x,x^{\prime})$ for any $x$ with fixed $x \in \mathcal{X}$, the kernelized stein discrepancy (KSD)~\cite{stein1,stein2,stein3} can be defined for measuring the difference between two distributions as below:
\begin{equation}
\mathbb{S}(q, p)=\max _{k(\cdot,x^{\prime}) \in \mathcal{H}^{d}}\left\{\left[\mathbb{E}_{x \sim q}\left(\operatorname{Tr}\left(\mathcal{A}_p k(x,x^{\prime})\right)\right)\right]^2, \quad \text { s.t. } \quad\|k(\cdot,x^{\prime})\|_{\mathcal{H}^d} \leq 1\right\},
\end{equation}
where the $\mathcal{A}_p k(x,x^{\prime})=k(x,x^{\prime}) \nabla_x \log p(x)^{\top}+\nabla_x k(x,x^{\prime})$ is the stein operator.
% 
And $\mathbb{S}(q, p)$ equals zero if and only if  $p(x)$ and $q(x)$ are the same.
% 




In the following, we compare \techname~with the existing two mainstream distribution-free estimation methods, i.e., score matching and MMD estimation, to analyze its effect and advance.
% 
On the one hand, score matching methods estimate probability densities without the need for distribution prior or distribution normalization~\cite{score_obj}, making it potential for generative task~\cite{ddpm}, statistical test~\cite{stein3} and variational inference~\cite{sm_vi}.
% 
However, score model estimates the density will inevitably fail once the distribution contains sparse data samples~\cite{ncsn,multiscale_score_ood1,ncsn} or multiple modalities~\cite{sm_multimodal_sampling}.
% 
% 
% Rethink the $L2-$norm of the score function, i.e., $\|s(x)\|= \|\nabla_{\boldsymbol{x}} \log p_t(\boldsymbol{x})\|=\|\frac{\nabla_{\boldsymbol{x}} p_t(\boldsymbol{x})}{p_t(\boldsymbol{x})}\|$, 
% it indicates that a high likelihood corresponds to a low norm and the semantic shift data will have high score norm due to its low density~\cite{multiscale_score_ood1}.\xenia{rewrite}
% 
On the other hand, MMD estimation accurately measures the distance between two densities in RKHS, which is competitive with three main strengths~\cite{mmd_pros1}, i.e., (1) it provides robust and consistent estimation, (2) it is insensitive in sample complexity, and (3) it employs a non-parametric implementation.
% 
% On the other hand, MMD estimation accurately measures the distance between two densities in RKHS and offers three competitive advantages, as outlined in \cite{mmd_pros1}: (1) it provides robust and consistent estimation, (2) it features favorable sample complexity, and (3) it employs a non-parametric implementation.
% alleviating unbiased estimation.
% 
Disappointingly, MMD matching has no efforts to enhance or correct the density estimation once the alignment distribution is unknown or inaccurate.




Recently, two prominent methods for unnormalized density estimation have emerged, i.e., score matching~\cite{score_obj} and MMD estimation~\cite{mmd1}. 
% 
Both approaches offer effectiveness but also come with inherent limitations.
% 
On the one hand, score matching methods estimate probability densities without the need for distribution prior or distribution normalization~\cite{score_obj}.
% , making it potential for generative task~\cite{ddpm}, statistical test~\cite{stein3} and variational inference~\cite{sm_vi}.
% 
However, score model estimates the density will inevitably fail once the distribution contains sparse data samples~\cite{ncsn,multiscale_score_ood1,ncsn} or multiple modalities~\cite{sm_multimodal_sampling}, as showing in Fig.~\ref{fig:toy_motivation} (a).


Rethink the $L2-$norm of the score function, i.e., $\|s(x)\|= \|\nabla_{\boldsymbol{x}} \log p_t(\boldsymbol{x})\|=\|\frac{\nabla_{\boldsymbol{x}} p_t(\boldsymbol{x})}{p_t(\boldsymbol{x})}\|$, 
it indicates that a high likelihood corresponds to a low norm and the semantic shift data will have high score norm due to its low density~\cite{multiscale_score_ood1}.\xenia{rewrite}

On the other hand, 
% MMD estimation accurately measures the distance between two densities in RKHS, which is competitive with three main strengths~\cite{mmd_pros1}, i.e., (1) it provides robust and consistent estimation, (2) it is insensitive in sample complexity, and (3) it employs a non-parametric implementation.
Conversely, 
MMD estimation accurately measures the distance between two densities in RKHS, showcasing three major advantages: robust and consistent estimation, insensitivity to sample complexity, and non-parametric implementation~\cite{mmd_pros1}.
% 
% On the other hand, MMD estimation accurately measures the distance between two densities in RKHS and offers three competitive advantages, as outlined in \cite{mmd_pros1}: (1) it provides robust and consistent estimation, (2) it features favorable sample complexity, and (3) it employs a non-parametric implementation.
% alleviating unbiased estimation.
% 
Disappointingly,  as depicting in Fig.~\ref{fig:toy_motivation} (d), MMD matching has no efforts to enhance or correct the density estimation once the alignment distribution is unknown or inaccurate.



% % 
Specifically, \techname~not only utilizes denoise score matching to capture the score between data samples and their close neighbors, but also explores the overall random data distribution, e.g., Normal distribution, via Langevin dynamic sampling from density vector fields modeled by score model.

Specifically, \techname~not only leverages denoise score matching to capture the scores between data samples and their proximate neighbors, while also investigating the broader random data distributions, such as the Normal distribution, through Langevin dynamic sampling from density vector fields modeled by the score model.


% 
\xenia{
Let $p_\sigma(\tilde{\boldsymbol{x}}| \boldsymbol{x}):=\mathcal{N}\left(\tilde{\boldsymbol{x}} ; \boldsymbol{x}, \sigma^2 \boldsymbol{I}\right)$ be a noise distribution, and  $p_\sigma(\tilde{\boldsymbol{x}}):=\int p_{\mathcal{D}}(\boldsymbol{x}) p_\sigma(\tilde{\boldsymbol{x}}|\boldsymbol{x}) \mathrm{d} \boldsymbol{x}$ denotes the estimated 
perturbed data distribution. 
% 
The noise conditional score network (NCSN)~\cite{ncsn} $\boldsymbol{s}_{\boldsymbol{\theta}}\left(\tilde{\boldsymbol{x}}, \sigma\right)$ is to minimize a weighted sum of denoising score matching~\cite{score_obj} as below:
\begin{equation}
\small
\begin{aligned}
% \boldsymbol{\theta}^*=\underset{\boldsymbol{\theta}}{\arg \min }
\ell(\boldsymbol{\theta}; \sigma) = \min \frac{1}{2}  \mathbb{E}_{p_{\mathcal{D}}(\boldsymbol{x})p_{\sigma}(\tilde{\boldsymbol{x}} \mid \boldsymbol{x})}\left\|\boldsymbol{s}_{\boldsymbol{\theta}}\left(\tilde{\boldsymbol{x}}, \sigma\right)-\nabla_{\tilde{\boldsymbol{x}}} \log p_{\sigma}(\tilde{\boldsymbol{x}} \mid \boldsymbol{x})\right\|_2^2.
\end{aligned}
\end{equation}
When the noise $\sigma \rightarrow 0$ , the optimal score model satisfies $\boldsymbol{s}_{\boldsymbol{\theta}^*}(\boldsymbol{x})=\nabla_{\boldsymbol{x}} \log q_\sigma(\boldsymbol{x}) \approx \nabla_{\boldsymbol{x}} \log p_{\mathcal{D}}(\boldsymbol{x})$.
% 
In practice, we prefer to explore a set of noise distribution with 
a positive geometric sequence, i.e., $\left\{\sigma_i\right\}_{i=1}^L=\left\{\frac{\sigma_1}{\sigma_2}=\ldots=\left(\frac{\sigma_{L-1}}{\sigma_{L}}\right)<1\right\}$, to obtain more robust score matching:
\begin{equation}
\mathcal{L} (\boldsymbol{\theta};\{\sigma_i\}^L_{i=1}) = \frac{1}{L} \sum^{L}_{i=1} \lambda (\sigma_i)\ell(\boldsymbol{\theta};\sigma_i).
\end{equation}
% 
Let $p(\boldsymbol{x})$ and $q(\boldsymbol{x})$ be a different smooth probability densities supported by $\boldsymbol{x}, \boldsymbol{x}^{\prime} \in\mathcal{X}$, and 
kernel function $k(\cdot, \cdot)$ belongs to the unit ball of a reproducing
kernel Hilbert space (RKHS) $\mathcal{H}$.
% , i.e., $k(x,x^{\prime})$ for any $x \in \mathcal{X}$ with fixed $x^{\prime} \in \mathcal{X}$.
}


\xenia{
% 
The maximum mean discrepancy (MMD) are defined as
% \begin{equation}
% \small
% \begin{aligned}
%     \operatorname{MMD}(\boldsymbol{p}, \boldsymbol{q})&=\sup _{\psi\in \mathcal{F}}\left(\mathbb{E}_{\boldsymbol{x}\sim \boldsymbol{p}}[\psi(\boldsymbol{x})]-\mathbb{E}_{\boldsymbol{y}\sim \boldsymbol{q}}[\psi(\boldsymbol{y})]\right)& = \sup _{\psi\in \mathcal{F} }\left(\frac{1}{M}\sum_{i=1}^{M}\psi(\boldsymbol{x}_i)-\frac{1}{N}\sum_{j=1}^{N}\psi(\boldsymbol{y}_j)\right).
% \end{aligned}
% \end{equation}

\begin{equation}
\begin{aligned}
     \operatorname{MMD}(\boldsymbol{p}, \boldsymbol{q})&=\sup _{k(\cdot,\cdot) \in \mathcal{H}^{d}}\left(\mathbb{E}_{\boldsymbol{x}\sim \boldsymbol{p}}[k(\boldsymbol{x},\boldsymbol{x})] -2\mathbb{E}_{\boldsymbol{x}\sim \boldsymbol{p},\boldsymbol{x}^{\prime}\sim \boldsymbol{q}}k(\boldsymbol{x},\boldsymbol{x}^{\prime}) +\mathbb{E}_{\boldsymbol{x}^{\prime}\sim \boldsymbol{q}}[k(\boldsymbol{x}^{\prime},\boldsymbol{x}^{\prime})]]\right).
\end{aligned}
\end{equation}
}
% 


% 
\xenia{Suppose a set of data samples $\{\boldsymbol{x} \in \mathbb{R}^{D}\}^N_{i=1}$ following unknown data distribution $p_{\mathcal{D}}(\boldsymbol{x})$, the score function of a probability density is defined as $\nabla_{\boldsymbol{x}} \log p_{\mathcal{D}}(\boldsymbol{x})$.
% 
The score model $\boldsymbol{s}_{\boldsymbol{\theta}} (\boldsymbol{x})$ is a neural network approximating score function $\nabla_{\boldsymbol{x}} \log p_{\mathcal{D}}(\boldsymbol{x})$.% with parameter $\boldsymbol{\theta}$.
% 
}
% 
The sampling iteration of \techname~can be defined as:
\begin{equation}
\begin{aligned}
\mathcal{L}_s & = \mathbb{E}_{p_{\mathcal{D}}(\boldsymbol{z}) p_{\sigma}(\tilde{\boldsymbol{z}} |\boldsymbol{z})}\left\|\boldsymbol{s}_{\boldsymbol{\theta}}\left(\tilde{\boldsymbol{z}}, \sigma\right)-\nabla_{\tilde{\boldsymbol{z}}} \log p_{\sigma}(\tilde{\boldsymbol{z}} \mid \boldsymbol{z})\right\|_2^2 +\lambda_{m}  
\operatorname{MMD}(\boldsymbol{z}, \boldsymbol{z}_{\text{gen})})
\end{aligned}
\label{eq:smd}
\end{equation}
where $\lambda_m$ is the trade-off coefficient, $p_{\mathcal{D}}(\boldsymbol{z})$ is the data distribution in latent representation space, 
$p_{\sigma}(\tilde{\boldsymbol{z}}| \boldsymbol{z})\sim \mathcal{N}(\boldsymbol{0},\sigma^2 \boldsymbol{I})$ is the noise-perturbed data distribution, ${\boldsymbol{z}}_{\text{gen}} =\boldsymbol{z}^T$ is the $T$-step short-cut MCMC  sampling from random noise $\boldsymbol{z}^0 \sim \mathcal{N}(\boldsymbol{0}, \boldsymbol{I})$:
\begin{equation}
\tilde{\boldsymbol{z}}^t=\tilde{\boldsymbol{z}}^{t-1}+\frac{\epsilon}{2} 
s_{\boldsymbol{\theta}}(\tilde{\boldsymbol{z}}^t,\sigma) + \sqrt{\epsilon} \boldsymbol{w}^t,
\label{eq:mcmc}
\end{equation}
with  $\boldsymbol{w}^t \sim \mathcal{N}(\boldsymbol{0}, \boldsymbol{I})$ denoting random noise in each step.




\subsection{Reliable Federated Density Estimation}
A reliable density distribution is eagerly necessary for distinguishing IN and OUT data~\cite{hanbo_ADL,DOS}.
%
In contrast to existing work that measures IN and OUT data distributions, 
 FL framework  is prevented from modeling ideal densities due to
the limitations in available OUT data and non-IID client data distributions.
% 
It becomes important to accurately capture the only visible IN distribution in each client, and further compose all client densities for a reliable global distribution.
% 
% But estimating free density without prior information is still challenging
% % 

In the following, we compare \techname~with the existing two mainstream distribution-free estimation methods, i.e., score matching and MMD estimation, to analyze its effect and advance.
% 
On the one hand, score matching methods estimate probability densities without the need for distribution prior or distribution normalization~\cite{score_obj}, making it potential for generative task~\cite{ddpm}, statistical test~\cite{stein3} and variational inference~\cite{sm_vi}.
% 
However, score model estimates the density will inevitably fail once the distribution contains sparse data samples~\cite{ncsn,multiscale_score_ood1,ncsn} or multiple modalities~\cite{sm_multimodal_sampling}.
% 
% 
% Rethink the $L2-$norm of the score function, i.e., $\|s(x)\|= \|\nabla_{\boldsymbol{x}} \log p_t(\boldsymbol{x})\|=\|\frac{\nabla_{\boldsymbol{x}} p_t(\boldsymbol{x})}{p_t(\boldsymbol{x})}\|$, 
% it indicates that a high likelihood corresponds to a low norm and the semantic shift data will have high score norm due to its low density~\cite{multiscale_score_ood1}.\xenia{rewrite}
% 
On the other hand, MMD estimation accurately measures the distance between two densities in RKHS, which is competitive with three main strengths~\cite{mmd_pros1}, i.e., (1) it leads to reliable and consistent estimation, (2) it requires lower sample complexity, and (3) it is non-parametric implementation.
% alleviating unbiased estimation.
% 
Disappointingly, MMD matching has no efforts to enhance or correct the density estimation once the alignment distribution is unknown or inaccurate.

\nosection{Local Density Estimation}
To reach this goal, we introduce a new density estimation framework \techname, which enjoys the advantages of existing density estimation methods, and brings an accurate and flexible implementation for federated scenarios.
% 
As shown in Fig.~\ref{fig:model}, in each client $k$, \techname~estimates data density in latent spaces, and holds a cooperative way between feature extractor $f_{\boldsymbol{\theta}}$ and density estimation $s_{{\boldsymbol{\theta}}}$.
% 
Specifically, given the latent representations $\boldsymbol{z}= f_{\boldsymbol{\theta}} (\boldsymbol{x})$, we first capture its density by modeling the score of \techname.
% 
Then \techname~regularize the feature extractor $f_{\boldsymbol{\theta}}$  based on the score values of latent representations $\nabla_{\boldsymbol{x}} \log p_{\boldsymbol{\theta}}(\boldsymbol{z})= s_{\boldsymbol{\theta}} (\boldsymbol{z})$ as a feedback regularization, except for the original loss of main task (e.g., cross entropy for classification).
% 





% 


This motivates us to design \techname~which explores the potential of connecting two density estimation paradigms.
% 
In this way, \techname~avoids the ineffectiveness of the above two methods, and enhances the density estimation by taking their advantages.
% 
Specifically, we not only utilize denoise score matching to capture the score between data samples and their close neighbors, but also encourage a Langevin sampling from a random distribution, e.g., $\boldsymbol{z}^0 \sim \mathcal{N}(\boldsymbol{0}, \boldsymbol{I})$, based on score model, which iterative generative sample neighbors of different distances simultaneously.
% 
The sampling iteration of \techname~can be defined as:
\begin{equation}
\small
\begin{aligned}
\mathcal{L}_s & = \mathbb{E}_{p_{\mathcal{D}}(\boldsymbol{z})p_{\sigma}(\tilde{\boldsymbol{z}} |\boldsymbol{z})}\left\|\boldsymbol{s}_{\boldsymbol{\theta}}\left(\tilde{\boldsymbol{z}}, \sigma\right)-\nabla_{\tilde{\boldsymbol{z}}} \log p_{\sigma}(\tilde{\boldsymbol{z}} \mid \boldsymbol{z})\right\|_2^2 +\\
&\lambda_{m}  \sup _{\psi\in \mathcal{F}}\left(\mathbb{E}_{ \boldsymbol{p}_{\mathcal{D}}}(\boldsymbol{z})[\psi(\boldsymbol{x})]-\mathbb{E}_{\boldsymbol{p}_{\boldsymbol{\theta}}(\hat{\boldsymbol{z}})}[\psi(\hat{\boldsymbol{z}})]\right)
% \left\|\int k(\boldsymbol{z}_{\text{gen}}, \boldsymbol{z}) \mathrm{d} \nu(\boldsymbol{z}_{\text{gen}})-\int k(\boldsymbol{z}_{\text{gen}}, \boldsymbol{z}) \mathrm{d} \mu(\boldsymbol{z})\right\|_{\mathcal{H}},
\end{aligned}
\label{eq:smd}
\end{equation}
where $\lambda_M$ is the trade-off coefficient, $p_{\mathcal{D}}(\boldsymbol{z})$ is the data distribution in latent representation space, 
$p_{\sigma}(\tilde{\boldsymbol{z}}| \boldsymbol{z})\sim \mathcal{N}(\boldsymbol{0},\sigma^2 \boldsymbol{I})$ is the noise-perturbed data distribution, $\hat{\boldsymbol{z}} =\boldsymbol{z}^T$ is the $T$-step short-cut MCMC  sampling from random noise  $\boldsymbol{z}^0 \sim \mathcal{N}(\boldsymbol{0}, \boldsymbol{I})$:
\begin{equation}
\tilde{\boldsymbol{z}}^t=\tilde{\boldsymbol{z}}^{t-1}+\frac{\epsilon}{2} 
s_{\boldsymbol{\theta}}(\tilde{\boldsymbol{z}}^t,\sigma) + \sqrt{\epsilon} \boldsymbol{w}^t,
\label{eq:mcmc}
\end{equation}
with  $\boldsymbol{w}^t \sim \mathcal{N}(\boldsymbol{0}, \boldsymbol{I})$ denoting random noise in each step.


% \begin{theorem}[Effective Score Matching]
% \xenia{similar equivalent proof}
% Assume that the estimated score function $s_{\boldsymbol{\theta}}(\boldsymbol{x})$ obeys the assumptions outlined in (Vincent, 2011), except that $s_{\boldsymbol{\theta}}(\boldsymbol{x})$ is instead differentiable almost everywhere. Then, the objective function for $\mathcal{J}_{E S M p}$ in (4) is still equivalent to $\mathcal{J}_{I S M p}$ in (5). Proof in Appendix B.4.
% \end{theorem}

\nosection{Motivation Example} 
% 
To illustrate the original motivation of \techname, we further visualize a density estimation of $2$-D toy example in Fig.~\ref{fig:toy_motivation}.
% 
In detail, we model the red scatters by tuning a series of coefficients, i.e., $\lambda_m=\{0, 0.1, 0.2, 0.5\}$ in Eq.~\eqref{eq:smd}.
% 
As we can see, with the calibration of MMD estimation, \techname~has more compact density estimation when $\lambda_m=0.5$, compared with blankly using score matching.
% 
% 
In the brand new objective of density estimation, \techname~expand the searching range and depth of score modeling, making it possible to comprehensively model data density.
% capture
% 
% 
Moreover, with the calibration of MMD estimation, original data representation and the generated latents based on the score model are effectively matched, bringing more realistic and correct estimation.
% 
Hence \techname~could ensure a more aligned and reliable density estimation for sparse and multi-modal data.


% 
\nosection{Global Densities Aggregation}
Given the local score models trained with Eq.~\eqref{eq:smd}, the server should compose all score models to obtain a reliable global density estimation.
% 
When \techname~approaches its optimality, i.e., $\boldsymbol{s}_{\boldsymbol{\theta}^*}(\boldsymbol{x})=\nabla_{\boldsymbol{z}} \log q_\sigma(\boldsymbol{z}) \approx \nabla_{\boldsymbol{z}} \log p_{\text {data }}(\boldsymbol{z})$, the density estimation can be formulated in the form of score model.
% 
Remind that score model is a parameterized neural model, making it adaptable for aggregation as conventional federated aggregations~\cite{FedAvg}, i.e.,
\begin{equation}
\{\boldsymbol{\theta}_s, \boldsymbol{\theta}_f\} = \sum_{k=1}^K p_k\{\boldsymbol{\theta}^k_s, \boldsymbol{\theta}^k_f\}
\label{eq:agg}
\end{equation}
with $p_k= \frac{\mathcal{D}_k}{\Sigma_{k=1}^{K} \mathcal{D}_k} , \forall_{k\in[K]}.$
% 
These collaborative processes among clients continue until the global model converges, bringing the reliable and comprehensive global density of all IN data.
% 


\begin{theorem}[Generalization Bound of \modelname]
\label{th:convergence}
Let assumptions \ref{supp_asu:l-lip}-\ref{supp_asu:bound_grad_norm} in appendix hold, and $L, \mu, \sigma_k, V$ be defined therein.
% 
Let $\kappa=\frac{L}{\mu}, \gamma=\max\{8\kappa, E\}$ and the learning rate $\eta_t=\frac{2}{\mu(\gamma+t)}$.
% 
The \modelname~with full client participation satisfies 
\begin{equation}
\small
\mathbb{E}\left[F\left({\overline{\boldsymbol{\theta}}}^t\right)\right]-F^* \leq \frac{\kappa}{\gamma+t}\left(\frac{2 B}{\mu}+\frac{\mu(\gamma+1)}{2} \|\boldsymbol{\theta}^t - \boldsymbol{\theta}^{*}\|^2\right),
\end{equation}
where $B=4(E-1)^2V^2 +K+2\Gamma$.


\end{theorem}









% The goal of \modelname~is to model a global score model with collaborative clients, enhancing the OOD detection and OOD generalization simultaneously.
% % 
% Specifically, we estimate the local in-distribution density by score models in each client, and aggregate these participating score models to generalize performance of diversifying covariate shift and enhance the semantic shift detection.
% 




% \subsection{Federated OOD Generalization and Detection}
% In this section, we first illustrate the main thoughts of the knowledge brought by density estimation, and then provide insights into tackling OOD generation and detection with estimated global density, respectively.
% % 
% In Fig.~\ref{fig:model}, we visualize a 2-dimensional score model in the form of vector field.
% % 
% For each vector in the vector field, its direction points to the high-density area, and its
% length indicates the distance from its position to the high-density area. 
% % 
% Once the local densities get well estimated, we can obtain the reliable global density of all IN data as a consistent indicator among all clients.
% % 

% \nosection{OOD detection in clients}
% % 
% It is evident that the larger the norm of score is, the more likely the data is OUT.
% % 
% That is, we have $\|\boldsymbol{s}_{\boldsymbol{\theta}^*}(\boldsymbol{z})\|=\|\nicefrac{\nabla_{\boldsymbol{x}} p_{\boldsymbol{\theta}}(\boldsymbol{z})}{ p_{\boldsymbol{\theta}}(\boldsymbol{z})}\|$ as the indicator of detecting OUT, i.e., 
% \begin{equation}
% g(\boldsymbol{s}_{\boldsymbol{\theta}} (\boldsymbol{z}))\left\{
% \begin{array}{cc}
%     0 & \|s_{\theta} (\boldsymbol{z})\| < \tau  \\
%     1 & otherwise.
% \end{array}
% \right.
% \end{equation}

% \xenia{\{}
% For evaluating the accuracy in Eq.~\eqref{eq:opt_goal}, we calibrate the prediction confidence for data samples via Eq.~\eqref{eq:g}, i.e., 
% \begin{equation}
% \tilde{\boldsymbol{y}} = \operatorname{Softmax}(\boldsymbol{l}/\|s_{\theta}(\boldsymbol{x})\|),
% \end{equation}
% where $\boldsymbol{l}$ is the original logits, and we enhance the detection performance by penalizing the high confidence of OUT data.

% \nosection{OOD generalization in clients}
% Given the score value, we define the Fisher information as $\mathcal{I} = \mathbb{E}_{\boldsymbol{x}\sim p_{\boldsymbol{\theta}}(\boldsymbol{x})} \left[\boldsymbol{s}_{\boldsymbol{\theta}^*}(\boldsymbol{x}) {\boldsymbol{s}_{\boldsymbol{\theta}^*}(\boldsymbol{x})^\top}\right]$, which measures the proximity between two examples $\boldsymbol{x}_1, \boldsymbol{x}_2$ in the model space~\cite{afv,jaakkola1998exploiting}.
% % 
% Thus we can define the score distance as:
% \begin{equation}
% \mathbb{D} (\boldsymbol{x}_1, \boldsymbol{x}_2) =  {\left(\boldsymbol{s}_{\boldsymbol{\theta}}(\boldsymbol{x}_1),  \boldsymbol{s}_{\boldsymbol{\theta}}(\boldsymbol{x}_2)\right)}^\top  \mathcal{I}^{-1} \left( {\boldsymbol{s}_{\boldsymbol{\theta}}(\boldsymbol{x}_1),  \boldsymbol{s}_{\boldsymbol{\theta}}(\boldsymbol{x}_2)}\right).
% \label{eq:g}
% \end{equation}
% This motivates us to regularize the feature extractor to learn more generalizable information based on the score distance in Eq.~\ref{eq:g}.
% % 
% During the model training, we optimize the feature extractor with main task loss and adversarial Fisher information:
% \begin{equation}
% \mathcal{L}_f = \mathcal{L}_{\textbf{ce}} + \lambda_g \mathbb{D}(\boldsymbol{z}, \boldsymbol{z}+\boldsymbol{\delta}), s.t., \boldsymbol{\delta} \in \mathbb{B}(\boldsymbol{z}, \boldsymbol{\delta}),
% \label{eq:feature_model}
% \end{equation}
% where $\mathbb{B}(\boldsymbol{z}, \boldsymbol{\delta})$ is the $l_\infty$ norm-ball around $\boldsymbol{z}$ with radius $\epsilon >0$.

% \begin{theorem}[Covariate shift generalization]
    
% \end{theorem}


Recently, two prominent methods for non-normalized density estimation have emerged, i.e., score matching~\cite{score_obj,score_reg_condition} and MMD estimation~\cite{mmd1,mmd_gen1}. 
% 
Both are effective but have inherent limitations. 
% 
Score matching estimates probability densities without requiring prior distribution knowledge or normalization~\cite{score_obj}, yet struggles with sparse data samples~\cite{ncsn,multiscale_score_ood1,ncsn} or multiple modalities~\cite{sm_multimodal_sampling}, as showing in Fig.~\ref{fig:toy_motivation} (a).
% 
In contrast, MMD estimation accurately measures the distance between two densities in RKHS, with the advantages of reliable and consistent estimation, insensitivity to sample complexity, and non-parametric implementation~\cite{mmd_pros1}.
% 
Unfortunately, as depicting in Fig.~\ref{fig:toy_motivation} (d), MMD matching does not enhance or correct density estimation when the alignment distribution is unknown or inaccurate.


% This has motivated us to develop \techname, which seeks to harness and integrate the strengths of both density estimation paradigms.
% % 
% In this way, \techname~brings an accurate and flexible implementation for federated scenarios.
% % 
% As shown in Fig.~\ref{fig:model}, in each client $k$, \techname~estimates data density in latent spaces, and holds a cooperative way between feature extractor $f_{\boldsymbol{\theta}}$ and score model $s_{{\boldsymbol{\theta}}}$.
% % 
% Thereby, given the latent representations $\boldsymbol{z}= f_{\boldsymbol{\theta}} (\boldsymbol{x})$, we first capture its density by modeling the score of \techname.
% 
Specifically, \techname~utilizes denoise score matching to accurately capture the scores between data samples and their nearby perturbed neighbors. 

Firstly, \techname~utilizes DSM to capture the local score function of latent features around its noise perturbed neighbors.
% 
Furthermore, the model broadly explores the whole space of random data distributions, such as the Normal distribution, e.g., $\boldsymbol{z}^0 \sim \mathcal{N}(\boldsymbol{0}, \boldsymbol{I})$. 
% 
It utilizes $T$-step Langevin dynamic sampling from density vector fields, as modeled by the score model, to derive generated latents $\boldsymbol{z}_{\text{gen}} = \boldsymbol{z}^T$:
\begin{equation}
{\boldsymbol{z}}^t={\boldsymbol{z}}^{t-1}+\frac{\epsilon}{2} 
s_{\boldsymbol{\theta}}({\boldsymbol{z}}^t,\sigma) + \sqrt{\epsilon} \boldsymbol{w}^t,
\label{eq:mcmc}
\end{equation}
with  $\boldsymbol{w}^t \sim \mathcal{N}(\boldsymbol{0}, \boldsymbol{I})$ denoting random noise in each step.
% 

Thus the sampling iteration of \techname~can be defined as:
\begin{equation}
\small
\begin{aligned}
\mathcal{L}_s & = \mathbb{E}_{p_{\mathcal{D}}(\boldsymbol{z}) p_{\sigma}(\tilde{\boldsymbol{z}} |\boldsymbol{z})}\left\|\boldsymbol{s}_{\boldsymbol{\theta}}\left(\tilde{\boldsymbol{z}}, \sigma\right)-\nabla_{\tilde{\boldsymbol{z}}} \log p_{\sigma}(\tilde{\boldsymbol{z}} \mid \boldsymbol{z})\right\|_2^2 +\lambda_{m}  
 \sup _{\psi\in \mathcal{F}}\left(\mathbb{E}_{ \boldsymbol{p}_{\mathcal{D}}}(\boldsymbol{z})[\psi(\boldsymbol{z})]-\mathbb{E}_{\boldsymbol{p}_{\boldsymbol{\theta}}({\boldsymbol{z}}_{\text{gen}})}[\psi(\boldsymbol{z}_{\text{gen}})]\right)
\end{aligned}
\label{eq:smd}
\end{equation}
where $\lambda_m$ is the trade-off coefficient, $p_{\mathcal{D}}(\boldsymbol{z})$ is the data distribution in latent feature space, 
$p_{\sigma}(\tilde{\boldsymbol{z}}| \boldsymbol{z})\sim \mathcal{N}(\boldsymbol{0},\sigma^2 \boldsymbol{I})$ is the noise-perturbed data distribution, and $\mathcal{F}$ as a set of functions: $\psi: \mathcal{X} \rightarrow \mathbb{R}$  within a unit ball in the universal Reproducing Kernel Hilbert Space $\mathcal{H}$ (RKHS) with norm $\|.\|_{\mathcal{H}}$.
% 


Stein identities, equations, and operators Stein's method [Stein, 1972] provides an elegant tool to characterise distributions via Stein operators, which can be used to assess distances between probability distributions, see for example Barbour and Chen [2005]. Mijoule et al. [2021]. Given a distribution $q$, an operator $\mathcal{A}_q$ is called a Stein operator w.r.t. $q$ and Stein class $\mathcal{F}$ if the following Stein identity holds for any test function $f \in \mathcal{F}: \mathbb{E}_q\left[\mathcal{A}_q f\right]=0$. For a test function $h$ one then aims to find a function $f=f_h \in \mathcal{F}$ which solves the Stein equation
$$
\mathcal{A}_q f(x)=h(x)-\mathbb{E}_q[h(x)] .
$$

Then for any distribution $p$, taking expectations $\mathbb{E}_p$ in Eq. 1 assesses the distance $\left|\mathbb{E}_p h-\mathbb{E}_q h\right|$ through $\left|\mathbb{E}_p \mathcal{A}_q f\right|$, an expression in which randomness enters only through the distribution $p$.
When the density function $q$ is given explicitly, with smooth support $\Omega_q \subset \mathbb{R}^m$, is differentiable and vanishes at the boundary of $\Omega_q$, a common choice of Stein operator in the literature is based on the
2
score-function $\mathrm{s}_q=\nabla \log q$ (with the convention that $\mathrm{s}_q \equiv 0$ outside of $\Omega_q$ ), see for example Mijoule et al. [2021]. Here, $\nabla$ denotes the gradient operator and taken to be a column vector. The score-Stein operator ${ }^1$ is the vector-valued operator acting on (vector-valued) function $\mathrm{f}$,
$$
\mathcal{A}_q \mathbf{f}(\boldsymbol{x})=\mathbf{f}(\boldsymbol{x})^{\top} \nabla \log q(\boldsymbol{x})+\nabla \cdot \mathbf{f}(\boldsymbol{x})
$$
and the Stein identity $\mathbb{E}_q\left[\mathcal{A}_q f\right]=0$ holds for functions $f$ which belong to the so-called canonical Stein class defined in Mijoule et al. [2021], Definition 3.2. As it requires knowledge of the density $q$ only via its score function, this Stein operator is particularly useful for unnormalised densities [Hyvärinen, 2005], appearing e.g. in energy based models (EBM) [LeCun et al., 2006].

Kernel Stein discrepancy To assess discrepancies between two probability distributions $p$ and $q$, the Stein discrepancy (w.r.t. class $\mathcal{B} \subset \mathcal{F}$ ) is defined as [Gorham and Mackey, 2015]
$$
\operatorname{SD}(p \| q, \mathcal{B})=\sup _{f \in \mathcal{B}}\{|\mathbb{E}_p\left[\mathcal{A}_q f\right]-\underbrace{\mathbb{E}_p\left[\mathcal{A}_p f\right]}_{=0}|\}=\sup _{f \in \mathcal{B}}\left|\mathbb{E}_p\left[\mathcal{A}_q f\right]\right| .
$$

As the $\sup f$ over a general class $\mathcal{B}$ can be difficult to compute, taking $\mathcal{B}$ as the unit ball of a reproducing kernel Hilbert space (RKHS) has been suggested in Chwialkowski et al. [2016], Liu et al. [2016], resulting in the kernel Stein discrepancy (KSD) defined as
$$
\operatorname{KSD}(p \| q, \mathcal{H})=\sup _{f \in \mathcal{B}_1(\mathcal{H})}\left|\mathbb{E}_p\left[\mathcal{A}_q f\right]\right| .
$$

Denoting by $k$ the reproducing kernel associated with the RKHS $\mathcal{H}$ over a set $\mathcal{X}$, the reproducing property ensures that $\forall f \in \mathcal{H}, f(\boldsymbol{x})=\langle f, k(\boldsymbol{x}, \cdot)\rangle_{\mathcal{H}}, \forall \boldsymbol{x} \in \mathcal{X}$. Algebraic manipulations yield
$$
\operatorname{KSD}^2(q \| p)=\mathbb{E}_{\boldsymbol{x}, \tilde{\boldsymbol{x}} \sim p}\left[u_q(\boldsymbol{x}, \tilde{\boldsymbol{x}})\right]
$$
where $u_q(\boldsymbol{x}, \tilde{\boldsymbol{x}})=\left\langle\mathcal{A}_q k(\boldsymbol{x}, \cdot), \mathcal{A}_q k(\tilde{\boldsymbol{x}}, \cdot)\right\rangle_{\mathcal{H}}$, which takes the exact sup without approximation and does not involve the (sample) distribution $p$. Then, $\mathrm{KSD}^2$ can be estimated through empirical means, over samples from $p$. For example, V-statistics [Van der Vaart, 2000] and U-statistics [Lee, 1990] estimates are
$$
\operatorname{KSD}_v^2(q \| p)=\frac{1}{m^2} \sum_{i, j} u_q\left(x_i, x_j\right), \quad \operatorname{KSD}_u^2(q \| p)=\frac{1}{m(m-1)} \sum_{i \neq j} u_q\left(\boldsymbol{x}_i \boldsymbol{x}_j\right) .
$$

KSD has been proposed as discrepancy measure between distributions for testing model goodness-offit in Chwialkowski et al. [2016] and Liu et al. [2016].

% \begin{wraptable}{L}{0.49\linewidth}
% % \begin{table}[]
% \centering
% \caption{OOD Detection comparison results on other OUT Data.}
% \label{tb:ood_detect}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{lcc|cc|cc|cc}
% \toprule
% OUT Data  & \multicolumn{2}{c}{LSUN-C} & \multicolumn{2}{c}{Place365} & \multicolumn{2}{c}{LSUN-R} & \multicolumn{2}{c}{Texture} \\
% \hline
%   Method    &  FPR95$\downarrow$ & AUROC$\uparrow$ &  FPR95$\downarrow$ & AUROC$\uparrow$ & FPR95$\downarrow$ & AUROC$\uparrow$ & FPR95$\downarrow$ & AUROC$\uparrow$ \\
% \hline
% FedAvg        &    62.10              &       76.29      &        80.02       &       62.14       &       62.01       &       77.02      &      80.53        &      66.23        \\
% FedLN  &       66.41           &       76.03      &         70.95      &      76.82        &       61.31       &      78.34       &       93.90       &        71.99      \\
% FedATOL   &  61.01 &  80.05  &  85.39 &  82.17 &  64.01 &  79.89 & 66.33 & 78.77 \\
% % FedT3A &                  &             &               &              &              &             &              &              \\
% FedIIR        &         57.86         &      77.98       &        83.68       &       64.04       &      58.44        &      78.69       &       91.72       &        62.32      \\
% \rowcolor{lightgray}
% FedAvg+\modelname  &       \textbf{  37.55 }        &     \textbf{ 91.22    }   &       \textbf{ 44.59}       &      \textbf{ 87.63 }      &     \textbf{ 44.16  }      &      \textbf{90.16 }      &    \textbf{  28.60  }      &        \textbf{ 91.75}     \\
% \midrule
% FedRoD   &        43.40          &       82.83      &        40.72       &      83.55        &       41.80       &       82.92      &       53.24       &     81.52         \\
% FOSTER  &        48.73          &        76.29     &       39.55        &      83.07        &       48.09       &      76.24       &        54.23      &        77.62      \\
% FedTHE &          43.72        &       83.50      &       39.22        &       85.95       &       42.95       &       83.46      &       53.58       &       82.19       \\
% FedICON  &         49.98         &      82.95       &        34.94       &        85.56      &        49.05      &       83.30      &       51.57       &        80.96      \\
% \rowcolor{lightgray}
% FedRoD+\modelname  & \textbf{36.17} &\textbf{  88.69}&   \textbf{17.61} & \textbf{ 94.56} &   \textbf{41.46} &   \textbf{92.80} &  \textbf{19.46} & \textbf{93.39}
%        \\

% \bottomrule
% \end{tabular}
% }
% \end{wraptable}
% % \end{table}
% \begin{wrapfigure}{r}{0.46\textwidth}
% \vspace{-16pt}
% \begin{center}
% \includegraphics[width=0.3\textwidth]{figs/in-c_generalization/CIFAR100_alpha0.1_ACC-IN-C.pdf}
% \end{center}
% \vspace{-8pt}
% \caption{The average results for Cifar100-C ($\alpha=0.1$) generalization.}
% \label{fig:inc_gen_avg}
% \vspace{-10pt}
% \end{wrapfigure}


% \begin{wrapfigure}{L}{\textwidth}
%     \begin{minipage}{0.45\textwidth}
%         \centering
%         \begin{tabular}{lcc|cc|cc|cc}
% \toprule
% OUT Data  & \multicolumn{2}{c}{LSUN-C} & \multicolumn{2}{c}{Place365} & \multicolumn{2}{c}{LSUN-R} & \multicolumn{2}{c}{Texture} \\
% \hline
%   Method    &  FPR95$\downarrow$ & AUROC$\uparrow$ &  FPR95$\downarrow$ & AUROC$\uparrow$ & FPR95$\downarrow$ & AUROC$\uparrow$ & FPR95$\downarrow$ & AUROC$\uparrow$ \\
% \hline
% FedAvg        &    62.10              &       76.29      &        80.02       &       62.14       &       62.01       &       77.02      &      80.53        &      66.23        \\
% FedLN  &       66.41           &       76.03      &         70.95      &      76.82        &       61.31       &      78.34       &       93.90       &        71.99      \\
% FedATOL   &  61.01 &  80.05  &  85.39 &  82.17 &  64.01 &  79.89 & 66.33 & 78.77 \\
% % FedT3A &                  &             &               &              &              &             &              &              \\
% FedIIR        &         57.86         &      77.98       &        83.68       &       64.04       &      58.44        &      78.69       &       91.72       &        62.32      \\
% \rowcolor{lightgray}
% FedAvg+\modelname  &       \textbf{  37.55 }        &     \textbf{ 91.22    }   &       \textbf{ 44.59}       &      \textbf{ 87.63 }      &     \textbf{ 44.16  }      &      \textbf{90.16 }      &    \textbf{  28.60  }      &        \textbf{ 91.75}     \\
% \midrule
% FedRoD   &        43.40          &       82.83      &        40.72       &      83.55        &       41.80       &       82.92      &       53.24       &     81.52         \\
% FOSTER  &        48.73          &        76.29     &       39.55        &      83.07        &       48.09       &      76.24       &        54.23      &        77.62      \\
% FedTHE &          43.72        &       83.50      &       39.22        &       85.95       &       42.95       &       83.46      &       53.58       &       82.19       \\
% FedICON  &         49.98         &      82.95       &        34.94       &        85.56      &        49.05      &       83.30      &       51.57       &        80.96      \\
% \rowcolor{lightgray}
% FedRoD+\modelname  & \textbf{36.17} &\textbf{  88.69}&   \textbf{17.61} & \textbf{ 94.56} &   \textbf{41.46} &   \textbf{92.80} &  \textbf{19.46} & \textbf{93.39}\\
% \bottomrule
% \end{tabular}
%     \end{minipage}
%     \begin{minipage}{0.45\textwidth}
% \includegraphics[width=0.43\textwidth]{figs/in-c_generalization/CIFAR100_alpha0.1_ACC-IN-C.pdf}
% \vspace{-8pt}
% \caption{The average results for Cifar100-C ($\alpha=0.1$) generalization.}
% \label{fig:inc_gen_avg}
% \vspace{-10pt}
% \end{minipage}
% % \caption{A wrapped table example with two columns.}
% \end{wrapfigure}


Considering the expectation of $q(x)$ on the Stein operator with score of $p(x)$, 
% $\mathbb{E}_{x \sim q(x)} \left[\mathcal{A}_{p(x)} h(x)\right] = \mathbb{E}_{x \sim q(x)} \left[\mathcal{A}_{p(x)} h(x)\right] - \mathbb{E}_{x \sim q(x)} \left[\mathcal{A}_{q(x)} h(x)\right]$, 
\begin{equation}
\begin{aligned}
\label{equ:norm}
\mathbb{E}_{x \sim q(x)} \left[\mathcal{A}_{p(x)} h(x)\right] &= \mathbb{E}_{x \sim q(x)} \left[\mathcal{A}_{p(x)} h(x)\right] - \mathbb{E}_{x \sim q(x)} \left[\mathcal{A}_{q(x)} h(x)\right] \\
& = \mathbb{E}_{x \sim q(x)} \left[\mathcal{A}_{p(x)} h(x) - \mathcal{A}_{q(x)} h(x)\right] \\
& = \mathbb{E}_{x \sim q(x)} \left[h(x) \left( \nabla \log p(x) - \nabla \log q(x)\right)\right]
\end{aligned}
\end{equation}
% https://arxiv.org/pdf/1909.13035#page=15.60

\begin{lemma}[Score Matching Equivalence]
% Given $\mathcal{D}= \mathcal{D}_1 \cup \cdots\cup \mathcal{D}_K$, we have the probability distribution $p(\mathcal{D})= p(\mathcal{D}_1 \cup \cdots\cup \mathcal{D}_K)= p(\mathcal{D}_1)\cdots p(\mathcal{D}_K)$ with the mild assumption that $p(\mathcal{D}_1), \cdots, p(\mathcal{D}_K) $ are independent.
% % 
% The error bound for modeling decentralized score models in clients is bounded similarly with the global bound by 
% \begin{equation}
% a=b+tbc
% \end{equation}
% \begin{proof}
% Given $\mathcal{D}= \mathcal{D}_1 \cup \cdots\cup \mathcal{D}_K$, we have the probability distribution $p(\mathcal{D})= p(\mathcal{D}_1 \cup \cdots\cup \mathcal{D}_K)= p(\mathcal{D}_1)\cdots p(\mathcal{D}_K)$ with the mild assumption that $p(\mathcal{D}_1) \cdots p(\mathcal{D}_K) $ are independent.
% Then the score function of golbal data can be written as:
% \begin{equation}
% \begin{aligned}
% \nabla_{\boldsymbol{x}} \log p_{\mathcal{D}} (\boldsymbol{x})& = \nabla_{\boldsymbol{x}} \log p_{\mathcal{D}_1} (\boldsymbol{x}) p_{\mathcal{D}_2} (\boldsymbol{x}) \cdots p_{\mathcal{D}_K} (\boldsymbol{x}) \\
% & = \nabla_{\boldsymbol{x}} \sum^K_{k=1} \log p_{\mathcal{D}_k}(\boldsymbol{x})\\
% &=   \sum^K_{k=1} \nabla_{\boldsymbol{x}} \log p_{\mathcal{D}_k}(\boldsymbol{x})\\
% \end{aligned}
% \end{equation}
\begin{proof}
Similarly, the global score model is aggregated from local score models that estimate the local IN data probability densities, i.e., $p_{\boldsymbol{\theta}^*_1}(\boldsymbol{x}) =p_{\mathcal{D}_1}(\boldsymbol{x}), \cdots, p_{\boldsymbol{\theta}^*_K}(\boldsymbol{x}) = p_{\mathcal{D}_K}(\boldsymbol{x})$
% 
This makes the below equation holds:
% \begin{equation}
% \begin{aligned}
% \nabla_{\boldsymbol{x}} \log p_{\boldsymbol{\theta}} (\boldsymbol{x})& = \nabla_{\boldsymbol{x}} \log p_{\boldsymbol{\theta}_1} (\boldsymbol{x}) p_{\boldsymbol{\theta}_2} (\boldsymbol{x}) \cdots p_{\boldsymbol{\theta}_K} (\boldsymbol{x}) \\
% & = \nabla_{\boldsymbol{x}} \sum^K_{k=1} \log p_{\boldsymbol{\theta}_k}(\boldsymbol{x})\\
% &=  \sum^K_{k=1} \nabla_{\boldsymbol{x}} \log p_{\boldsymbol{\theta}_k}(\boldsymbol{x})\\
% \end{aligned}
% \end{equation}
\begin{equation}
\begin{aligned}
 \nabla_{\boldsymbol{x}} \log p_{\boldsymbol{\theta}} (\boldsymbol{x})=s_{\boldsymbol{\theta}}(\boldsymbol{x})&=\sum^K_{k=1} w_k s_{\boldsymbol{\theta}_k}(\boldsymbol{x})\\
   &=  \sum^K_{k=1} w_k \nabla_{\boldsymbol{x}} \log p_{\boldsymbol{\theta}_k}(\boldsymbol{x})\\
 & = \nabla_{\boldsymbol{x}} \sum^K_{k=1}  w_k\log p_{\boldsymbol{\theta}_k}(\boldsymbol{x})\\
  % & = \nabla_{\boldsymbol{x}} \log p_{\boldsymbol{\theta}_1} (\boldsymbol{x}) p_{\boldsymbol{\theta}_2} (\boldsymbol{x}) \cdots p_{\boldsymbol{\theta}_K} (\boldsymbol{x}) \\
% 
%  & = \nabla_{\boldsymbol{x}} \log p_{\boldsymbol{\theta}_1} (\boldsymbol{x}) p_{\boldsymbol{\theta}_2} (\boldsymbol{x}) \cdots p_{\boldsymbol{\theta}_K} (\boldsymbol{x}) \\
% & = \nabla_{\boldsymbol{x}} \sum^K_{k=1} \log p_{\boldsymbol{\theta}_k}(\boldsymbol{x})\\
% &=  \sum^K_{k=1} \nabla_{\boldsymbol{x}} \log p_{\boldsymbol{\theta}_k}(\boldsymbol{x})\\
\end{aligned}
\end{equation}

we obtain the global score function by  model $s_{\boldsymbol{\theta}}(\cdot)$ 
Then we formulate the score matching for global distribution as 
\begin{equation}
\begin{aligned}
    &\|\nabla_{\boldsymbol{x}} \log p_{\boldsymbol{\theta}}(\boldsymbol{x}) - \nabla_{\boldsymbol{x}} \log p_{\mathcal{D}} (\boldsymbol{x})\|^2\\
    &= \| \sum^K_{k=1} w_k \nabla_{\boldsymbol{x}} \log p_{\boldsymbol{\theta}_k}(\boldsymbol{x})- \nabla_{\boldsymbol{x}} \log p_{\mathcal{D}} (\boldsymbol{x})\|^2\\
    &= \| \sum^K_{k=1} w_k \nabla_{\boldsymbol{x}} \log p_{\boldsymbol{\theta}_k}(\boldsymbol{x})- \sum^K_{k=1} w_k \nabla_{\boldsymbol{x}} \log p_{\mathcal{D}} (\boldsymbol{x})\|^2\\
    &= \|\sum^K_{k=1} w_k [ \nabla_{\boldsymbol{x}} \log p_{\boldsymbol{\theta}_k}(\boldsymbol{x})- \nabla_{\boldsymbol{x}} \log p_{\mathcal{D}} (\boldsymbol{x})]\|^2\\
    & \leq \sum^K_{k=1} w_k \| \nabla_{\boldsymbol{x}} \log p_{\boldsymbol{\theta}_k}(\boldsymbol{x})- \nabla_{\boldsymbol{x}} \log p_{\mathcal{D}} (\boldsymbol{x})\|^2\\
    % &= \sum^K_{k=1} w_k \| \nabla_{\boldsymbol{x}} \log p_{\boldsymbol{\theta}_k}(\boldsymbol{x})-  \sum^K_{k=1} \nabla_{\boldsymbol{x}} \log p_{\mathcal{D}_k}(\boldsymbol{x})\|^2\\
    % &= \sum^K_{k=1} w_k \| \sum^K_{k=1} \frac{1}{K} \nabla_{\boldsymbol{x}} \log p_{\boldsymbol{\theta}_k}(\boldsymbol{x})-  \sum^K_{k=1} \nabla_{\boldsymbol{x}} \log p_{\mathcal{D}_k}(\boldsymbol{x})\|^2
\end{aligned}
\end{equation}
\end{proof}
\end{lemma}


==> chapters/theory.tex <==
\section{Priliminaries}
Suppose a set of data samples $\{\boldsymbol{x} \in \mathbb{R}^{\mathcal{D}}\}^N_{i=1}$ following unknown data distribution $p_{\mathcal{D}}(\boldsymbol{x})$, the score function of a probability density is defined as $\nabla_{\boldsymbol{x}} \log p_{\mathcal{D}}(\boldsymbol{x})$.
% 
The score model $\boldsymbol{s}_{\boldsymbol{\theta}} (\boldsymbol{x})$ is a neural network approximating score function $\nabla_{\boldsymbol{x}} \log p_{\mathcal{D}}(\boldsymbol{x})$.% with parameter $\boldsymbol{\theta}$.
% 




\subsection{Denoise Score Matching and Langevin Dynamics Inference}
Let $p_\sigma(\tilde{\boldsymbol{x}}| \boldsymbol{x}):=\mathcal{N}\left(\tilde{\boldsymbol{x}} ; \boldsymbol{x}, \sigma^2 \boldsymbol{I}\right)$ be a noise distribution, and  $p_\sigma(\tilde{\boldsymbol{x}}):=\int p_{\mathcal{D}}(\boldsymbol{x}) p_\sigma(\tilde{\boldsymbol{x}}|\boldsymbol{x}) \mathrm{d} \boldsymbol{x}$ denotes the estimated 
perturbed data distribution. 
% 
The noise conditional score network (NCSN)~\cite{ncsn} $\boldsymbol{s}_{\boldsymbol{\theta}}\left(\tilde{\boldsymbol{x}}, \sigma\right)$ is to minimize a weighted sum of denoising score matching~\cite{score_obj} as below:
\begin{equation}
\small
\begin{aligned}
% \boldsymbol{\theta}^*=\underset{\boldsymbol{\theta}}{\arg \min }
\ell(\boldsymbol{\theta}; \sigma) = \min \frac{1}{2}  \mathbb{E}_{p_{\mathcal{D}}(\boldsymbol{x})p_{\sigma}(\tilde{\boldsymbol{x}} \mid \boldsymbol{x})}\left\|\boldsymbol{s}_{\boldsymbol{\theta}}\left(\tilde{\boldsymbol{x}}, \sigma\right)-\nabla_{\tilde{\boldsymbol{x}}} \log p_{\sigma}(\tilde{\boldsymbol{x}} \mid \boldsymbol{x})\right\|_2^2.
\end{aligned}
\end{equation}
When the noise $\sigma \rightarrow 0$ , the optimal score model satisfies $\boldsymbol{s}_{\boldsymbol{\theta}^*}(\boldsymbol{x})=\nabla_{\boldsymbol{x}} \log q_\sigma(\boldsymbol{x}) \approx \nabla_{\boldsymbol{x}} \log p_{\mathcal{D}}(\boldsymbol{x})$.
% 
In practice, we prefer to explore a set of noise distribution with 
a positive geometric sequence, i.e., $\left\{\sigma_i\right\}_{i=1}^L=\left\{\frac{\sigma_1}{\sigma_2}=\ldots=\left(\frac{\sigma_{L-1}}{\sigma_{L}}\right)<1\right\}$, to obtain more robust score matching:
\begin{equation}
\mathcal{L} (\boldsymbol{\theta};\{\sigma_i\}^L_{i=1}) = \frac{1}{L} \sum^{L}_{i=1} \lambda (\sigma_i)\ell(\boldsymbol{\theta};\sigma_i)
\end{equation}
% 
% 
Once the score model converges to its optimal parameter $\boldsymbol{\theta}^*$, we can substitute the data score function for sampling and inference.
% 
% 
Specifically, $T$-steps of Langevin dynamics sampling can generate samples from the score model of $p_{\mathcal{D}}(x)$ with step size $\epsilon>0$ as below:
\begin{equation}
\tilde{\boldsymbol{x}}^t=\tilde{\boldsymbol{x}}^{t-1}+\frac{\epsilon}{2} \boldsymbol{s}_{\boldsymbol{\theta}^*}(\boldsymbol{x}) +\sqrt{\epsilon} \boldsymbol{z}^t,
\end{equation}
where $\boldsymbol{z}^t \sim \mathcal{N}(0, I)$ is added to avoid collapse, and $\boldsymbol{x}^0$ can be sampled by a prior distribution, e.g., $\boldsymbol{x}^0 \sim \mathcal{N}\left(\boldsymbol{x}|\boldsymbol{0}, \sigma^2 \boldsymbol{I}\right)$.
% 
% 
 The distribution of $\tilde{\boldsymbol{x}}^T$ equals $p(\boldsymbol{x})$ when $\epsilon \rightarrow 0$ and $T \rightarrow \infty$, where $\tilde{\boldsymbol{x}}^T$ becomes an exact sample from $p_{\mathcal{D}}(\boldsymbol{x})$ under some regularity conditions~\cite{score_reg_condition}.
% 
% Therefore, in order to obtain samples from $p_{\text {data }}(\boldsymbol{x})$, we can first train our score network such that $\boldsymbol{s}_{\boldsymbol{\theta}}(\boldsymbol{x}) \approx \nabla_{\boldsymbol{x}} \log p_{\text {data }}(\boldsymbol{x})$ and then approximately obtain samples with Langevin dynamics using $\boldsymbol{s}_{\boldsymbol{\theta}}(\boldsymbol{x})$. This is the key idea of our framework of score-based generative modeling.




\subsection{Maximum Mean Discrepancy and Kernelized Stein Discrepancy}
Let $p(\boldsymbol{x})$ and $q(\boldsymbol{x})$ be a different smooth probability densities supported by $\boldsymbol{x}, \boldsymbol{x}^{\prime} \in\mathcal{X}$, and 
kernel function $k(\cdot, \cdot)$ belongs to the unit ball of a reproducing
kernel Hilbert space (RKHS) $\mathcal{H}$.
% , i.e., $k(x,x^{\prime})$ for any $x \in \mathcal{X}$ with fixed $x^{\prime} \in \mathcal{X}$.
% 
The maximum mean discrepancy (MMD) are defined as
% \begin{equation}
% \small
% \begin{aligned}
%     \operatorname{MMD}(\boldsymbol{p}, \boldsymbol{q})&=\sup _{\psi\in \mathcal{F}}\left(\mathbb{E}_{\boldsymbol{x}\sim \boldsymbol{p}}[\psi(\boldsymbol{x})]-\mathbb{E}_{\boldsymbol{y}\sim \boldsymbol{q}}[\psi(\boldsymbol{y})]\right)& = \sup _{\psi\in \mathcal{F} }\left(\frac{1}{M}\sum_{i=1}^{M}\psi(\boldsymbol{x}_i)-\frac{1}{N}\sum_{j=1}^{N}\psi(\boldsymbol{y}_j)\right).
% \end{aligned}
% \end{equation}

\begin{equation}
\begin{aligned}
     \operatorname{MMD}(\boldsymbol{p}, \boldsymbol{q})&=\sup _{k(\cdot,\cdot) \in \mathcal{H}^{d}}\left(\mathbb{E}_{\boldsymbol{x}\sim \boldsymbol{p}}[k(\boldsymbol{x},\boldsymbol{x})] -2\mathbb{E}_{\boldsymbol{x}\sim \boldsymbol{p},\boldsymbol{x}^{\prime}\sim \boldsymbol{q}}k(\boldsymbol{x},\boldsymbol{x}^{\prime}) +\mathbb{E}_{\boldsymbol{x}^{\prime}\sim \boldsymbol{q}}[k(\boldsymbol{x}^{\prime},\boldsymbol{x}^{\prime})]]\right).
\end{aligned}
\end{equation}

% 
The kernelized stein discrepancy (KSD)~\cite{stein1,stein2,stein3} can be defined for measuring the difference between two distributions as below:
\begin{equation}
\mathbb{S}(q, p)=\max _{k(\cdot,x^{\prime}) \in \mathcal{H}^{d}}\left\{\left[\mathbb{E}_{x \sim q}\left(\operatorname{Tr}\left(\mathcal{A}_p k(x,x^{\prime})\right)\right)\right]^2, \quad \text { s.t. } \quad\|k(\cdot,x^{\prime})\|_{\mathcal{H}^d} \leq 1\right\},
\end{equation}
where the $\mathcal{A}_p k(x,x^{\prime})=k(x,x^{\prime}) \nabla_x \log p(x)^{\top}+\nabla_x k(x,x^{\prime})$ is the stein operator.
% 
And $\mathbb{S}(q, p)$ equals zero if and only if  $p(x)$ and $q(x)$ are the same.
% 



